Solving Phase Retrieval with a Learned Reference

Fourier phase retrieval is a classical problem that deals with the recovery of an image from the amplitude measurements of its Fourier coefficients. Conventional methods solve this problem via iterative (alternating) minimization by leveraging some prior knowledge about the structure of the unknown image. The inherent ambiguities about shift and flip in the Fourier measurements make this problem especially difficult; and most of the existing methods use several random restarts with different permutations. In this paper, we assume that a known (learned) reference is added to the signal before capturing the Fourier amplitude measurements. Our method is inspired by the principle of adding a reference signal in holography. To recover the signal, we implement an iterative phase retrieval method as an unrolled network. Then we use back propagation to learn the reference that provides us the best reconstruction for a fixed number of phase retrieval iterations. We performed a number of simulations on a variety of datasets under different conditions and found that our proposed method for phase retrieval via unrolled network and learned reference provides near-perfect recovery at fixed (small) computational cost. We compared our method with standard Fourier phase retrieval methods and observed significant performance enhancement using the learned reference.

==> definitions.tex <==
\usepackage{graphicx}
\usepackage{amsmath,amsfonts,amsthm,amssymb,xspace,bm, verbatim,dsfont}
\usepackage{url,algorithm,algpseudocode}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{cleveref}
\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing,angles,quotes}
\usetikzlibrary{positioning,plotmarks,calc}
\usepackage{bbm}
\usepackage{todonotes}
\usepackage{subfig}
\usepackage{pgfplots}
  
%% Theorems, Lemmas, Proofs, Definitions %%
%\theoremstyle{plain}
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{definition}[theorem]{Definition}

%% Notes %%
\theoremstyle{definition}
\newcommand{\note}[1]{\marginpar{\tiny *note in TeX*}}
%% Operators %%

%Probability%
\DeclareMathOperator*{\pr}{\mathsf{Pr}}
\newcommand{\prob}[1]{\mathbb{P}\left[#1\right]}
\DeclareMathOperator*{\ex}{\mathbb{E}}
\newcommand{\expec}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\normal}{\mathcal{N}(0,1)}
\newcommand{\gauss}{\mathcal{N}}

%Real and Complex spaces
\newcommand{\rn}{\mathbb{R}^n}
\newcommand{\rnn}{\mathbb{R}^{n \times n}}
\newcommand{\rmm}{\mathbb{R}^{m \times m}}
\newcommand{\rmn}{\mathbb{R}^{m \times n}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\complex}{\mathbb{C}}

%Identity and ones
\newcommand{\eye}{\mathbb{I}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\ones}{\mathbbm{1}}

%Vectors and Matrices%
\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}

%Matrix operations - Trace, Rank, Norms, Inner products
\newcommand{\iprod}[2]{\left\langle #1, #2 \right\rangle} 
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\phase}[1]{\mathrm{Ph}\left(#1\right)}
\newcommand{\conj}[1]{\overline{#1}}
\newcommand{\imag}[1]{\textrm{Im}\left(#1\right)}

%\newcommand{\norm}[1]{{\left\lVert{#1}\right\rVert}}
\newcommand{\frob}[1]{\left\| {#1} \right\|_\text{F}}
\newcommand{\zeronorm}[1]{\left\| {#1} \right\|_0}
\newcommand{\onenorm}[1]{\left\| {#1} \right\|_1}
\newcommand{\twonorm}[1]{\left\| {#1} \right\|_2}
\newcommand{\infnorm}[1]{\left\| {#1} \right\|_{\infty}}

\newcommand{\sign}[1]{\operatorname{sign}\left(#1\right)}
\newcommand{\Tr}{\operatorname{Tr}}
\DeclareMathOperator{\trace}{Tr}

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\dist}[2]{\|#1-#2\|_2}
\newcommand{\distop}[2]{\mathrm{dist}\left(#1,#2\right)}

%Sets
\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\newcommand{\supp}[1]{\operatorname{supp}(#1)}
%\DeclareMathOperator*{\argmin}{argmin}
%\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\card}[1]{\operatorname{card}(#1)}
\newcommand{\trunc}[1]{\operatorname{trunc}(#1)}

%Complexity
\newcommand{\order}[1]{\mathcal{O}\left({#1}\right)}
\newcommand{\ordereps}[1]{\mathcal{O}_{\epsilon}\left({#1}\right)}
%Brackets
\newcommand{\rbrak}[1]{\left(#1\right)}
\newcommand{\sbrak}[1]{\left[#1\right]}
\newcommand{\cbrak}[1]{\left\{#1\right\}}
\newcommand{\sqfr}[2]{\sqrt{\frac{#1}{#2}}}
\newcommand{\frsq}[2]{\frac{#1}{\sqrt{#2}}}

%Paper-specific variables%
%\newcommand{\eps}{\epsilon}
\newcommand{\y}{\vect{y}}
\newcommand{\e}{\vect{e}}
\newcommand{\z}{\vect{z}}
\newcommand{\w}{\vect{w}}
\newcommand{\uu}{\vect{u}}
\newcommand{\rr}{\vect{r}}
\newcommand{\vv}{\vect{v}}
\newcommand{\zhat}{\hat{\z}}
\newcommand{\xo}{\vect{x^*}}
\newcommand{\xin}{\vect{x^0}}
%\newcommand{\x}{\vect{x}}
\newcommand{\xt}{\x^t}
\newcommand{\xtplus}{\x^{t+1}}
\newcommand{\xplus}{\x^+}
\newcommand{\xtilde}{\vect{\widetilde{x}}}
\newcommand{\xSmin}{\x_{S_{-}}^*}
\newcommand{\xSpls}{{\x_{S_{+}}^*}}
\newcommand{\xSbmin}{\x_{S_{b-}}^*}
\newcommand{\xSbpls}{{\x_{S_{b+}}^*}}
\newcommand{\xShat}{{\x_{\hat{S}}^*}}
\newcommand{\xSbhat}{{\x_{\hat{S_b}}^*}}
\newcommand{\xS}{\x_{S}^*}
\newcommand{\ai}{\vect{a}_i}
\newcommand{\aiS}{{\ai_{S}}}
\newcommand{\aiShat}{{\ai}_{\hat{S}}}
\newcommand{\aiSmin}{\ai_{S_{-}}}
\newcommand{\aiSpls}{\ai_{S_{+}}}
\renewcommand{\P}{\mat{P}}
\newcommand{\p}{\vect{p}}
\newcommand{\h}{\vect{h}}
\newcommand{\A}{\mat{A}}
\newcommand{\D}{\mat{D}}
\newcommand{\M}{\mat{M}}
\newcommand{\U}{\mat{U}}
\newcommand{\subspaces}{{\mathcal{M}}}


%\newcommand{\red}[1]{\textcolor{red}{#1}}
%\newcommand{\blue}[1]{\textcolor{blue}{#1}}

%\newcommand{\tikzmark}[1]{\tikz[overlay,remember picture] \node (#1) {};}
%
%\newcommand*{\AddNote}[4]{%
%	\begin{tikzpicture}[overlay, remember picture]
%	\draw [decoration={brace,amplitude=0.5em},decorate,ultra thick,red]
%	($(#3)!(#1.north)!($(#3)-(0,1)$)$) --  
%	($(#3)!(#2.south)!($(#3)-(0,1)$)$)
%	node [align=center, text width=2.5cm, pos=0.5, anchor=west] {#4};
%	\end{tikzpicture}
%}%

\newcommand{\sinc}{\mathrm{sinc}}
\newcommand{\mA}{\ensuremath{\mathbf A}}
\newcommand{\mB}{\ensuremath{\mathbf B}}
\newcommand{\mE}{\ensuremath{\mathbf E}}
\newcommand{\mF}{\ensuremath{\mathbf F}}
\newcommand{\mG}{\ensuremath{\mathbf G}}
\newcommand{\mL}{\ensuremath{\mathbf L}}
\newcommand{\mM}{\ensuremath{\mathbf M}}
\newcommand{\mQ}{\ensuremath{\mathbf Q}}
\newcommand{\mR}{\ensuremath{\mathbf R}}
\newcommand{\mS}{\ensuremath{\mathbf S}}
\newcommand{\mT}{\ensuremath{\mathbf T}}
\newcommand{\mU}{\ensuremath{\mathbf U}}
\newcommand{\mV}{\ensuremath{\mathbf V}}
\newcommand{\mW}{\ensuremath{\mathbf W}}
\newcommand{\mX}{\ensuremath{\mathbf X}}
\newcommand{\mY}{\ensuremath{\mathbf Y}}
\newcommand{\mZ}{\ensuremath{\mathbf Z}}
\newcommand{\ve}{\ensuremath{\mathbf e}}
\newcommand{\va}{\ensuremath{\mathbf a}}
\newcommand{\vb}{\ensuremath{\mathbf b}}
\newcommand{\vc}{\ensuremath{\mathbf c}}
\newcommand{\vf}{\ensuremath{\mathbf f}}
\newcommand{\vg}{\ensuremath{\mathbf g}}
\newcommand{\vh}{\ensuremath{\mathbf h}}
\newcommand{\vp}{\ensuremath{\mathbf p}}
\newcommand{\vr}{\ensuremath{\mathbf r}}
\newcommand{\vs}{\ensuremath{\mathbf s}}
\newcommand{\vu}{\ensuremath{\mathbf u}}
%\newcommand{\vv}{\ensuremath{\mathbf v}}
\newcommand{\vw}{\ensuremath{\mathbf w}}
\newcommand{\vx}{\ensuremath{\mathbf x}}
\newcommand{\vy}{\ensuremath{\mathbf y}}
\newcommand{\vz}{\ensuremath{\mathbf z}}
\newcommand{\vpsi}{\ensuremath{\mathbf \psi}}
\newcommand{\vphi}{\ensuremath{\mathbf \phi}}
\newcommand{\ct}{\ensuremath{\widetilde{c}}}
\newcommand{\setT}{\ensuremath{\mathcal T}}
\newcommand{\proj}{\ensuremath{\mathcal P}}
\newcommand{\rf}[1]{\ensuremath{{\mathbf \phi}_{#1}}}
\newcommand{\af}[1]{\ensuremath{\underline{\mathbf f}_{#1}}}
\newcommand{\ru}[1]{\ensuremath{{\mathbf u}_{#1}}}
\newcommand{\qa}[1]{\ensuremath{\hat{a}_{#1}}}
\newcommand{\comp}[2]{\ensuremath{c_{#1,#2}}}
\newcommand{\resid}[2]{\ensuremath{\vr_{#1,#2}}}
\newcommand{\cerr}[2]{\ensuremath{\ct_{#1,#2}}}
\newcommand{\vsW}{\ensuremath{\mathcal{W}}}
\newcommand{\vsS}{\ensuremath{\mathcal{S}}}
\newcommand{\vsH}{\ensuremath{\mathcal{H}}}
\newcommand{\opF}{\ensuremath{\mathbf{F}}}
\newcommand{\piF}{\ensuremath{\mathbf{F}^\dagger}}
\newcommand{\adjF}{\ensuremath{\mathbf{F}^*}}
\newcommand{\Epsilon}{\ensuremath{\mathcal{E}}}
\newcommand{\Reals}{\ensuremath{\mathbb{R}}}
\newcommand{\SD}{\ensuremath{\Sigma\Delta}}
\newcommand{\MMSE}{\ensuremath{\mbox{MMSE}}}
%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\dvec}{\bf vec}
%\DeclareMathOperator{\sign}{sign}
%\DeclareMathOperator{\diag}{diag}
%\newcommand{\supp}[1]{\ensuremath{\operatorname{supp}\left(#1\right)}}
\newcommand{\diag}[1]{\ensuremath{\operatorname{diag}\left(#1\right)}}
\newcommand{\nullsp}[1]{\ensuremath{\operatorname{null}(#1)}}
\newcommand{\range}[1]{\ensuremath{\operatorname{range}(#1)}}
\renewcommand{\dim}[1]{\ensuremath{\operatorname{dim}(#1)}}
\newcommand{\spanof}[1]{\ensuremath{\operatorname{span}\{#1\}}}
\newcommand{\rankof}[1]{\ensuremath{\operatorname{rank}\{#1\}}}
%\newcommand{\qed}{\framebox{}}
\newtheorem{Theorem}{Theorem}
\newtheorem{Definition}{Definition}
\newtheorem{Lemma}{Lemma}
\newcommand{\PBnote}[1]{{\em [**PB:{#1}]}}
\newcommand{\Salnote}[1]{{\em [**SAL:{#1}]}}


\newcommand{\field}[1]{\mathbb{#1}}                                   % Topological sets
\newcommand{\prn}[1]{\left(#1\right)}                                 % Parenthetical
\newcommand{\Prn}[1]{\left[#1\right]}                                 % Parenthetical 2
\newcommand{\clog}[1]{\textnormal{Log}\left(#1\right)}                % Complex Logarithm
\newcommand{\cfn}[2]{#1\left(#2\right)}                               % Continuous function
\newcommand{\dfn}[2]{#1\left[#2\right]}                               % Discrete function
\newcommand{\dff}[2]{\displaystyle\frac{d#1}{d#2}}                    % Differential (fraction form)
\newcommand{\dfe}[2]{\displaystyle\frac{d}{d#2}\left(#1\right)}       % Differential (expression form)
\newcommand{\pdff}[2]{\displaystyle\frac{\partial #1}{\partial #2}}   % Partial Differential (fraction form)
\newcommand{\pdfe}[2]{\displaystyle\frac{\partial}{\partial #2}#1}    % Partial Differential (expression form)
\newcommand{\pdo}[1]{\displaystyle\frac{\partial}{\partial #1}}       % Partial Differential Operator
%dfrac:   \newcommand{\nfrac}[2]{\displaystyle\frac{#1}{#2}}                    % Display Fraction
\newcommand{\dlim}[2]{\displaystyle\lim_{#1}\left(#2\right)}          % Display Limit
\newcommand{\dint}[3]{\displaystyle\int_{#1}^{#2}{#3}}                % Display Integral
\newcommand{\dsum}[3]{\displaystyle\sum_{#1}^{#2}{#3}}                % Display Sum
\newcommand{\centerup}[1]{\begin{center}#1\end{center}}               % Center text
\newcommand{\HRule}{\rule{\linewidth}{0.5mm}}                         % Horizontal line
%\newcommand{\abs}[1]{\left|#1\right|}                                 % Absolute value
\newcommand{\elone}[1]{\left\|#1\right\|_1}                           % L-1 Norm
\newcommand{\eltwo}[1]{\left\|#1\right\|_2}                           % L-2 Norm
\newcommand{\elinf}[1]{\left\|#1\right\|_\infty}                      % L-infinity Norm
\newcommand{\fro}[1]{\left\|#1\right\|_{fro}}                         % Frobenius Norm
%\newcommand{\norm}[1]{\left\|#1\right\|}                              % Norm
\renewcommand{\labelenumi}{(\alph{enumi})}                            % To get enumerate to display letters
\newcommand{\ip}[1]{\langle{#1}\rangle}																 % Inner Product
\newcommand{\sarray}[1]{\begin{array}{l}#1\end{array}}								 % simple array
\newcommand{\sarrayc}[1]{\begin{array}{c}#1\end{array}}								 % simple array (center)
\newcommand{\darray}[1]{\begin{array}{ll}#1\end{array}}								 % double array
\newcommand{\darraycl}[1]{\begin{array}{cl}#1\end{array}}							 % double array (center,left)
\newcommand{\res}[1]{\centerup{\framebox{#1}}}												 % Important result (centered and boxed)
\newcommand{\amatrix}[1]{\begin{bmatrix}#1\end{bmatrix}}							 % matrix (bmatrix)
\newcommand{\minim}[2]{\underset{#1}{\min}{#2}}												 % minimize
\newcommand{\maxim}[2]{\underset{#1}{\max}{#2}}												 % maximize
%\newcommand{\sign}[1]{\mathrm{sign}{\left(#1\right)}}									 % sign function
%
% Theorems, Lemmas, Proposition...
%
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{proposition}{Proposition}[section]
%\newtheorem{definition}{Definition}[section]
%
% LCA Symbols
%
\newcommand{\G}{\Gamma}
\newcommand{\Gc}{\Gamma^c}
\newcommand{\g}{\gamma}
\newcommand{\PP}{\Phi_{\Gamma}^T\Phi_{\Gamma}}
\newcommand{\PcP}{\Phi_{\Gamma^c}^T\Phi_{\Gamma}}
%
% Custom Trig functions
%
\newcommand{\cosine}[1]{\mathbf{\cos}\left(#1\right)}
\newcommand{\sine}[1]{\mathbf{\sin}\left(#1\right)}
\newcommand{\cosinep}[2]{\mathbf{\cos}^{#2}\left(#1\right)}
\newcommand{\sinep}[2]{\mathbf{\sin}^{#2}\left(#1\right)}
\newcommand{\tangent}[1]{\tan\left(#1\right)}
\newcommand{\cosecant}[1]{\csc\left(#1\right)}
\newcommand{\secant}[1]{\sec\left(#1\right)}
\newcommand{\cotangent}[1]{\cot\left(#1\right)}
\newcommand{\arctangent}[1]{\tan^{-1}\left(#1\right)}
\newcommand{\arcsine}[1]{\arcsin\left(#1\right)}
\newcommand{\arccosine}[1]{\arccos\left(#1\right)}
\newcommand{\hypsine}[1]{\sinh\left(#1\right)}
\newcommand{\hypcosine}[1]{\cosh\left(#1\right)}
\newcommand{\hyptangent}[1]{\tanh\left(#1\right)}
\newcommand{\atanq}[2]{\arctangent{\gfrac{#1}{#2}}}
%
% Custom tabbing
%
\newcommand{\etab}{\ \ \ \ }
\newcommand{\dnl}{\newline\newline}                                  % Double newline
%
% Probability Functions
%
\newcommand{\expc}[1]{E\left[#1\right]}	                             % Expectation
\newcommand{\expco}[2]{E\left[\left.#1\right|#2\right]}              % Conditional Expectation
\newcommand{\exps}[2]{E_{#1}\left[#2\right]}                         % Expectation with subscript
\newcommand{\var}[1]{\texttt{var}\func{#1}}		                       % Variance
\newcommand{\vars}[2]{\texttt{var}_{#1}\func{#2}}                    % Variance with subscript
\newcommand{\cov}[1]{\texttt{cov}\func{#1}}		                       % Covariance
\newcommand{\pdf}[2]{\mkfunc{f_{#1}}{#2}}                            % Probability Distribution Function
%\newcommand{\pr}[1]{Pr\func{#1}} 						                         % Probability
%
% Probability Distributions
%
\newcommand{\gaussian}[1]{\dfrac{1}{\sqrt{2\pi\sigma_{#1}^2}}e^{-\frac{\prn{#1-\mu_{#1}}^2}{2\sigma_{#1}^2}}}
%
% Figure
%
\newcommand{\fig}[4]{\begin{figure}
\begin{center}
\includegraphics[width=#1]{#2}
\caption{#3}
\label{fig:#4}
\end{center}
\end{figure}}
%
\newcommand{\figh}[4]{\begin{figure}[h]
\begin{center}
\includegraphics[width=#1]{#2}
\caption{#3}
\label{fig:#4}
\end{center}
\end{figure}}

